Don't stop me now: How Validation Criteria Affect Checkpoint Selection and Early Stopping

Checkpoint selection is a standard component of neural network training, yet the validation criterion used to select a checkpoint is often chosen heuristically. Moreover, the same criterion may be used either only to rank checkpoints after completion of a predefined training run or also to determine when training should stop, thereby affecting both the selected checkpoint and the set of checkpoints available for selection. In this work, we systematically investigate the role of validation criteria under these two settings. We separately vary the training loss, the validation criterion, and the target evaluation metric, and compare post-hoc checkpoint selection, in which training proceeds for all predefined epochs, with patience-based early stopping, in which the validation criterion also controls training termination. We consider three Cross-Entropy, C-Loss, and PolyLoss as training losses, and accuracy, macro-F1, and Matthews correlation coefficient as target metrics. Selection quality is assessed through the relative gap between the test performance of the validation-selected checkpoint and the best-observed test performance for the same target metric over the complete predefined training run.

==> __FIG_GAPS.tex <==
\begin{figure}[p]
\centering
\includegraphics[
height=\textheight,
width=1.5\linewidth,
keepaspectratio
]{images/stripplot_relative_ce_training_acc.png}
\caption{Relative Accuracy gap on the tabular datasets for models trained using Cross-Entropy. The panels correspond to the different validation criteria, while colors indicate the parameterization ratio $r$.}
\label{fig:stripplot_ce_training_acc}
\end{figure}

\begin{figure}[p]
\centering
\includegraphics[
height=1.5\textheight,
width=1.2\linewidth,
keepaspectratio
]{images/stripplot_relative_closs_training_acc.png}
\caption{Relative Accuracy gap on the tabular datasets for models trained using C-Loss. The panels correspond to the different validation criteria, while colors indicate the parameterization ratio $r$.}
\label{fig:stripplot_closs_training_acc}
\end{figure}

\begin{figure}[p]
\centering
\includegraphics[
height=1.5\textheight,
width=1.2\linewidth,
keepaspectratio
]{images/stripplot_relative_polyloss_training_acc.png}
\caption{Relative Accuracy gap on the tabular datasets for models trained using PolyLoss. The panels correspond to the different validation criteria, while colors indicate the parameterization ratio $r$.}
\label{fig:stripplot_polyloss_training_acc}
\end{figure}



\begin{figure}[p]
\centering
\includegraphics[
height=1.5\textheight,
width=1.2\linewidth,
keepaspectratio
]{images/stripplot_relative_ce_training_f1_macro.png}
\caption{Relative macro-F1 gap on the tabular datasets for models trained using Cross-Entropy. The panels correspond to the different validation criteria, while colors indicate the parameterization ratio $r$.}
\label{fig:stripplot_ce_training_f1}
\end{figure}

\begin{figure}[p]
\centering
\includegraphics[
height=1.5\textheight,
width=1.2\linewidth,
keepaspectratio
]{images/stripplot_relative_closs_training_f1_macro.png}
\caption{Relative macro-F1 gap on the tabular datasets for models trained using C-Loss. The panels correspond to the different validation criteria, while colors indicate the parameterization ratio $r$.}
\label{fig:stripplot_closs_training_f1}
\end{figure}

\begin{figure}[p]
\centering
\includegraphics[
height=1.5\textheight,
width=1.2\linewidth,
keepaspectratio
]{images/stripplot_relative_polyloss_training_f1_macro.png}
\caption{Relative macro-F1 gap on the tabular datasets for models trained using PolyLoss. The panels correspond to the different validation criteria, while colors indicate the parameterization ratio $r$.}
\label{fig:stripplot_polyloss_training_f1}
\end{figure}

\textit{Finally, Figures~\ref{fig:stripplot_ce_training_mcc}--\ref{fig:stripplot_polyloss_training_mcc} report the corresponding results for MCC.}

\begin{figure}[p]
\centering
\includegraphics[
height=1.5\textheight,
width=1.2\linewidth,
keepaspectratio
]{images/stripplot_relative_ce_training_mcc.png}
\caption{Relative MCC gap on the tabular datasets for models trained using Cross-Entropy. The panels correspond to the different validation criteria, while colors indicate the parameterization ratio $r$.}
\label{fig:stripplot_ce_training_mcc}
\end{figure}

\begin{figure}[p]
\centering
\includegraphics[
height=1.5\textheight,
width=1.2\linewidth,
keepaspectratio
]{images/stripplot_relative_closs_training_mcc.png}
\caption{Relative MCC gap on the tabular datasets for models trained using C-Loss. The panels correspond to the different validation criteria, while colors indicate the parameterization ratio $r$.}
\label{fig:stripplot_closs_training_mcc}
\end{figure}

\begin{figure}[p]
\centering
\includegraphics[
height=1.5\textheight,
width=1.2\linewidth,
keepaspectratio
]{images/stripplot_relative_polyloss_training_mcc.png}
\caption{Relative MCC gap on the tabular datasets for models trained using PolyLoss. The panels correspond to the different validation criteria, while colors indicate the parameterization ratio $r$.}
\label{fig:stripplot_polyloss_training_mcc}
\end{figure}


\begin{figure}[p]
\centering
\includegraphics[
height=0.82\textheight,
width=\linewidth,
keepaspectratio
]{images/stripplot_image_datasets_acc.png}
\caption{Relative Accuracy gap on CIFAR-10 and TinyImageNet-200 using ResNet-50. The panels correspond to the validation criteria used for checkpoint selection, while colors identify the training loss.}
\label{fig:image_datasets_acc}
\end{figure}

\begin{figure}[p]
\centering
\includegraphics[
height=0.82\textheight,
width=\linewidth,
keepaspectratio
]{images/stripplot_image_datasets_f1_macro.png}
\caption{Relative macro-F1 gap on CIFAR-10 and TinyImageNet-200 using ResNet-50. The panels correspond to the validation criteria used for checkpoint selection, while colors identify the training loss.}
\label{fig:image_datasets_f1_macro}
\end{figure}

\begin{figure}[p]
\centering
\includegraphics[
height=0.82\textheight,
width=\linewidth,
keepaspectratio
]{images/stripplot_image_datasets_mcc.png}
\caption{Relative MCC gap on CIFAR-10 and TinyImageNet-200 using ResNet-50. The panels correspond to the validation criteria used for checkpoint selection, while colors identify the training loss.}
\label{fig:image_datasets_mcc}
\end{figure}


==> note.tex <==
\section{Related works}

loss function theorical studies: \citep{rosasco2004loss}

early stopping is also known with other names, such as "spotted minimization" \citep{sjoberg1995overtraining}

A first formal description of the overtraining phenomena is provided in \citep{wang1993optimal}. In \citep{dodier1995geometry}, a geometric characterization on early stopping in linear models is given. 
 
In \citep{baldi1991temporal}, the authors analytically study the temporal evolution of generalization in linear ANNs on quadratic loss, discussing the validation-error dynamics.

\citep{hagiwara2002regularization} proposed a statistical interpretation of regularization and early stopping  for the linear regression model. 



Several studies document the beneficial effects of early stopping in artificial neural networks (ANNs). The interesting work proposed in \citep{caruana2000overfitting} noticed that early stopping allows large neural networks to terminate training once they have converged to solutions comparable to those produced by optimally sized smaller networks. The efficacy of early stopping as an implicit regularizer for ANNs in particular conditions is also supported in \citep{ji2021early}.


\citep{bishop1995regularization} considers alternative strategies for controlling the complexity of feed-forward networks showing a connection between early stopping and regularization \citep{evgeniou2002regularization} for quadratic loss functions. In other words, early stopping can be viewed as a form o regularization "over time". Similar consideration were made also in \citep{sjoberg1995overtraining}.

\citep{natarajan1997automated} proposed an early-stopping scheme that augments a proposed stopping rule with an iteration-count term to handle spurious early steady-state plateaus attributed to premature neuron saturation, reporting no significant difference in predictive performance relative to standard stopping methods. Furthermore, the proposed method seems to be affect by severe data leakage \citep{} by resampling a validation set from the entire training data at every epoch.
The same method is also explored in \citep{iyer2000novel}.

More broadly, early-stopping schemes can be grouped into two categories \citep{ferro2023early}: (i) training-monitored rules, which track a quality metric on the training data; and (ii) validation-monitored rules, which assess performance on a held-out set distinct from the training data. For example, in \citep{ennett2003evaluation} the authors propose a log-sensitivity index as an early-stopping rule based on the training set loss for ANNs tackling rare outcomes.

\citep{prechelt2002early} empirically analyzes validation-monitored stopping rules for MLPs. In In \citep{nguyen2005stopping} three different early stopping criteria was experimented in the context of evolutionary ANNs. Other early stopping rules and their combination are benchmarked in \citep{lodwich2009} on classical ANNs classification tasks.

The loss surface of ANNs is discussed in several works, e.g. \citep{soudry2016no,swirszcz2016local,goodfellow2014qualitatively}.  


\citep{suliman2018early} simply stops the training when the error on the validation set is below a given threshold.
\citep{shao2010comparison} proposed to stop the training when the reduction of MSE between iterations became marginal, i.e. less than the learning rate. 

Rather than designing a loss-based stopping rule, \citep{wu2009new} frames early stopping around the hold-out protocol, focusing on how the train–validation split is constructed to monitor generalization.


In particular, the role of Cross Entropy and the squared loss in classification problems has been discussed in \citep{demirkaya2020exploring}.

\citep{lalis2014adaptive} discusses a stopping criteria relyed only on the training loss.


\citep{singh2014c} provided a loss function based on the Correntropy \citep{santamaria2006generalized}, a measure of statistical similarity based on the second and higher order statistics.
\citep{demirkaya2020exploring} proposed the Correct-Class-Quadratic Loss (CCQL), a regularized modification of the squared loss which put more emphasis on the correct class.


\citep{zhang2020penetrating} analyzed several regularization methods (including early stopping) and found that regularization shapes the representations learned in hidden layers; specifically, it seems that early stopping mitigates overfitting  reducing the injection of irrelevant information into hidden-layer encodings.

The authors of \citep{ferro2023early} proposed an early-stopping criterion that halts training when multiple online indicators become highly correlated over a sliding window.

\citep{miseta2024surpassing} proposed the Correlation-Driven Stopping Criterion (CDSC) which simultaneously monitors the model performance on the training and validation sets, stopping  the training process when the Pearson correlation between the training and validation losses decreases below a given threshold. 


Apart from the supervised learning for ANNs, other studies have considered the optimal stopping timing for different familes of ML models.
For instance, early stopping has been extensively addressed in the context of boosting methods, as discussed in works such as \citep{buhlmann2003boosting,barron2008approximation,chen2013learning,wei2017early}and SVMs \citep{bandos2007statistical}.
Several of these studies established consistency results for specific early stopping strategies, demonstrating that the statistical error of the resulting estimator vanishes asymptotically as the sample size grows \citep{wei2017early}.
